Tandem spoofing-robust automatic speaker verification based on time-domain embeddings

Spoofing-robust automatic speaker verification (SASV) systems are a crucial technology for the protection against spoofed speech. In this study, we focus on logical access attacks and introduce a novel approach to SASV tasks. A novel representation of genuine and spoofed speech is employed, based on the probability mass function (PMF) of waveform amplitudes in the time domain. This methodology generates novel time embeddings derived from the PMF of selected groups within the training set. This paper highlights the role of gender segregation and its positive impact on performance. We propose a countermeasure (CM) system that employs time-domain embeddings derived from the PMF of spoofed and genuine speech, as well as gender recognition based on male and female time-based embeddings. The method exhibits notable gender recognition capabilities, with mismatch rates of 0.94% and 1.79% for males and females, respectively. The male and female CM systems achieve an equal error rate (EER) of 8.67% and 10.12%, respectively. By integrating this approach with traditional speaker verification systems, we demonstrate improved generalization ability and tandem detection cost function evaluation using the ASVspoof2019 challenge database. Furthermore, we investigate the impact of fusing the time embedding approach with traditional CM and illustrate how this fusion enhances generalization in SASV architectures.

==> commands.tex <==
% \begin{table}[h]
% \caption{Comparison of EERs between the score fusion using time-embedding machine learning classifiers and the systems from \cite{zhang2021one} for males, females, and both genders.}
% \centering
% \begin{tabular}{lcc}
% \hline
% \textbf{Subset} & \textbf{System} &   \textbf{EER (\%)} \\ \hline
% Dev. & Fusion (Softmax+Time) &   0.00$^{0.00}_{0.00}$ / 0.00$^{0.03}_{0.00}$  /  0.00$^{0.02}_{0.00}$   \\
% Dev. & Fusion (AMSoftmax+Time) &   0.01$^{0.05}_{0.00}$ /  0.06$^{0.25}_{0.00}$ /  0.04$^{0.17}_{0.00}$  \\ 
% Dev. & Fusion (OC-Softmax+Time) &   0.08$^{2.32}_{2.00}$ /  0.03$^{0.08}_{0.00}$ /  0.05$^{0.09}_{0.00}$ \\ 
% Eval. & Fusion (Softmax+Time) &   3.71$^{4.49}_{3.12}$ / 4.80$^{5.57}_{4.03}$ / 4.47$^{5.11}_{3.92}$  \\
% Eval. & Fusion (AMSoftmax+Time) &    3.00$^{3.58}_{2.28}$ /  3.19$^{3.84}_{2.41}$ /  3.13$^{3.59}_{2.52}$  \\ 
% Eval. & Fusion (OC-Softmax+Time) &    2.13$^{2.59}_{1.67}$ /  1.98$^{2.57}_{1.47}$ /  2.02$^{2.42}_{1.64}$  \\ 

% \hline
% \end{tabular}
% \label{tab:CM_EER_fUSION}
% \end{table}

לעבור על הכותרת
על מה שמסומן בכחול

יכול להיות ערכים של alpha נוספים שנותנים את הביצועים האופטימליים ((זה קורה רק בסט הולידציה בסט הולידציה). כאשר זה מתקיים אז בחרתי את הalpha  הנמוך ביותר, ועדיין ההפרש בינו לבין הסט מבחן גבוהה - כלומר המסקנה שלנו עדיין מתקיימת.

ועל התקציר
